General Cops and Robbers Games with randomness

Cops and Robbers games have been studied for the last few decades in computer science and mathematics. As in general pursuit evasion games, pursuers (cops) seek to capture evaders (robbers); however, players move in turn and are constrained to move on a discrete structure, usually a graph, and know the exact location of their opponent. In 2017, Bonato and MacGillivray presented a general characterization of Cops and Robbers games in order for them to be globally studied. However, their model doesn't cover cases where stochastic events may occur, such as the robbers moving in a random fashion. In this paper we present a novel model with stochastic elements that we call a Generalized Probabilistic Cops and Robbers game (GPCR). A typical such game is one where the robber moves according to a probabilistic distribution, either because she is rather lost or drunk than evading, or because she is a robot. We present results to solve GPCR games, thus enabling one to study properties relating to the optimal strategies in large classes of Cops and Robbers games. Some classic Cops and Robbers games properties are also extended.

==> HeadersAndCommands.tex <==
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\makeatletter
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}

\newcommand{\coprob}{Cops and Robbers}
\newcommand{\expth}{\textrm{EXPTIME-hard}}
\newcommand{\exptc}{\textrm{EXPTIME-complete}}
\newcommand{\NPC}{\textrm{NP-complete}}
\newcommand{\NPH}{\textrm{NP-hard}}
\newcommand{\pspaceh}{\textrm{PSPACE-hard}}
\newcommand{\pspace}{\textrm{PSPACE}}


\newcommand{\robbers}{\mathrm{rob}}
\newcommand{\petitsrobbers}{\scalebox{0.7}{\rm rob}}%pour avoir plus petit et mieux espacé en indice
\newcommand{\cops}{\mathrm{cop}}
\newcommand{\petitscops}{\scalebox{0.7}{\rm cop}}
\newcommand{\objects}{\mathrm{o}}
\newcommand{\x}{\textsf{x}}
\newcommand{\ic}{i_{\petitscops}}
\newcommand{\ir}{i_{\petitsrobbers}}
\newcommand{\stc}{S_{\petitscops}}
\newcommand{\str}{S_{\petitsrobbers}}
\newcommand{\sto}{S_{\objects}}
\newcommand{\ac}{A_{\petitscops}}
\newcommand{\ar}{A_{\petitsrobbers}}
\newcommand{\tc}{T_{\petitscops}}
\newcommand{\tr}{T_{\petitsrobbers}}
\newcommand{\acs}[1]{A_{\petitscops}(#1)}
\newcommand{\ars}[1]{A_{\petitsrobbers}(#1)}
\newcommand{\cac}{a_{\petitscops}}
\newcommand{\rac}{a_{\petitsrobbers}}
\newcommand{\acopt}{a_{\petitscops}^*}
\newcommand{\aropt}{a_{\petitsrobbers}^*}
\newcommand{\tx}{T_{\x}}
\newcommand{\ax}{A_{\x}}
\newcommand{\axs}[1]{A_{\x}(#1)}

\newcommand{\strcset}{\Omega_{\cops}}
\newcommand{\strrset}{\Omega_{\robbers}}
\newcommand{\strcsetfini}{\Omega^{\mathrm {f}}_{\cops}}
\newcommand{\strrsetfini}{\Omega^{\mathrm {f}}_{\robbers}}
\newcommand{\strc}{\sigma_{\cops}}
\newcommand{\strr}{\sigma_{\robbers}}
\newcommand{\ctime}{T_{\scalebox{0.8}{$\strc, \strr$}}}%ceci pour que les indices soient plus beau quant à l'espacement
\newcommand{\pn}{p_n^*}
\newcommand{\ptime}[1]{p_{#1}^*}
\newcommand{\pg}{p_\game^*}

\newcommand{\sw}{\overline{w}}

\newcommand{\game}{\cl{G}}
\newcommand{\parcours}{P_{(s, a^*)}^F}
\newcommand{\ggame}{\cl{H}}

\newcommand{\pcopnsym}[1]{c_p^{#1}(\mathcal{G})}
\newcommand{\pcopntext}[1]{$(p,#1)$-cop number}
\newcommand{\pcopsym}{c_p(\mathcal{G})}
\newcommand{\pcoptext}{$p$\textrm{-cop number}}

\newcommand{\win}{\textrm{copwin}}
\newcommand{\cwin}[1]{$c(1,#1)$\textrm{-win}}
\newcommand{\cpwin}[1]{$c(p,#1)$\textrm{-win}}
\newcommand{\cpnwin}[2]{$c(#1,#2)$\textrm{-win}}
\newcommand{\pcopwin}{$p$\textrm{-\win{}}}

\newcommand{\jail}{j^*}

\newcommand{\pt}[1]{\cl{P}_{#1}}
\newcommand{\pth}[2]{\cl{P}_{#1}^{#2}}

\newcommand{\dist}[1]{\mathrm{Dist}_{#1}}
\newcommand{\unif}[1]{\mathcal{U}_{#1}}
\newcommand{\dirac}[1]{\delta_{#1}}


\newcommand{\hiye}[1]{\colorbox{yellow}{#1}}
\newcommand{\p}[1]{\mathbb{P}\left[#1\right]}
\newcommand{\e}[1]{\mathbb{E}\left[#1\right]}

\newcommand{\bigO}[1]{\mathop{}\!O{\left(#1\right)}}
\newcommand{\smallO}[1]{\mathop{}\!o{\left(#1\right)}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\se}[1]{\left\{#1\right\}}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\note}[2][orange!80]{
\todo[inline, color=#1]{{#2}}
}
\newcommand{\cl}[1]{\mathcal{#1}}

\newcommand{\optVal}[3]{p_{#1}^*(#2, #3)}
\newcommand*{\var}{\makebox[1ex]{\textbf{$\cdot$}}}%

\newcommand{\nodef}{
	\includegraphics[scale=0.035]{bowen_knot.png}
}
